New Insights on the Stokes Paradox for Flow in Unbounded Domains

Stokes flow equations, used to model creeping flow, are a commonly used simplification of the Navier--Stokes equations. The simplification is valid for flows where the inertial forces are negligible compared to the viscous forces. In infinite domains, this simplification leads to a fundamental paradox. In this work we review the Stokes paradox and present new insights related to recent research. We approach the paradox from three different points of view: modern functional analysis, numerical simulations, and classical analytic techniques. The first approach yields a novel, rigorous derivation of the paradox. We also show that relaxing the Stokes no-slip condition (by introducing a Navier's friction condition) in one case resolves the Stokes paradox but gives rise to d'Alembert's paradox. The Stokes paradox has previously been resolved by Oseen, who showed that it is caused by a limited validity of Stokes' approximation. We show that the paradox still holds for the Reynolds--Orr equations describing kinetic energy flow instability, meaning that flow instability steadily increases with domain size. We refer to this as an instability paradox.

==> machip_siam.tex <==
\newcommand{\kef}{{\mathcal E}}
\newcommand{\bigA}{{\bf A}}
\newcommand{\bigB}{{\bf B}}
\newcommand{\tmp}[1]{{\times 10^{-{#1}}}}
\newcommand{\dtx}[1]{{\frac{\partial^2\phantom{#1}}{\partial #1^2}}}
\newcommand{\dpx}[1]{{\frac{\partial\phantom{#1}}{\partial #1}}}
\newcommand{\dpt}[2]{{\frac{\partial^2\phantom{#1}}{{\partial #1}{\partial #2}}}}
\newcommand{\betac}{b}
\newcommand{\hx}{\hat x}
\newcommand{\hk}{\hat k}
\newcommand{\hl}{\hat l}
\newcommand{\xdk}{\langle\hx,\hk\rangle}
\newcommand{\eixk}{e^{\iota \xdk}}
\newcommand{\ery}{e^{-(\rho y)^2}}
\newcommand{\eryt}{e^{-2(\rho y)^2}}
\newcommand{\pol}{\mathcal{P}}
\newcommand{\exitau}{\mathcal{T}}
\newcommand{\Omh}{\Omega_h}
\newcommand{\Th}{\mathcal{T}_h}
\newcommand{\btau}{{\boldsymbol \tau}}
\newcommand{\omitit}[1]{}
\newcommand{\Reyuls}{\mathbb{R}}
\newcommand{\ntegrs}{\mathbb{Z}}
\newcommand{\Rp}{{\mathbb{R}_+}}
\newcommand{\Rtwo}{\mathbb{R}^2}
\newcommand{\Rtre}{\mathbb{R}^3}
\newcommand{\Rdee}{\mathbb{R}^d}
\newcommand{\Rn}{\mathbb{R}^n}
%newcommand{\P}{{{\rm I}{\relax\ifmmode\mskip-\thinmuskip\relax\else\kern-.19667em\fi}{\bf P}}}
\newcommand{\p}{{{\rm I}{\relax\ifmmode\mskip-\thinmuskip\relax\else\kern-.22em\fi}{\bf P}}}
\newcommand{\perpzh}{\perp\kern-.20em^a}

\newcommand{\Plang}{{\p}{\kern-.03em{\rm fortran}}}
%\newcommand{\Pfortran}{{\p}{\rm fortran}}
\newcommand{\Pfortran}{{\p}{\kern-.03em{\rm fortran}}}
\newcommand{\pfortran}{{\Pfortran}}
\newcommand{\plang}{{\Pfortran}}
%%%%%%%% draft size for 12 point
%\setlength{\textheight}{8.7in}
%\setlength{\textwidth}{6.5in}
%\addtolength{\topmargin}{-0.5in}
%\setlength{\oddsidemargin}{+.0in}
%\setlength{\evensidemargin}{-.0in}
%%%%%%%% draft size 
\setlength{\textheight}{8.0in}
\setlength{\textwidth}{5.5in}
\addtolength{\topmargin}{-0.0in}
%for viewing only
%\setlength{\oddsidemargin}{-.5in}
%\setlength{\evensidemargin}{-.5in}
\setlength{\oddsidemargin}{.5in}
\setlength{\evensidemargin}{.5in}

\newcommand{\odim}{d}

\newcommand{\half}{{\textstyle{1\over 2}}}
\newcommand{\third}{{\textstyle{1\over 3}}}
\newcommand{\fourth}{{\textstyle{1\over 4}}}
\newcommand{\twelfth}{{\textstyle{1\over 12}}}
\newcommand{\twothirds}{{\textstyle{2\over 3}}}
\newcommand{\threehalfs}{{\textstyle{3\over 2}}}

\newcommand{\Forall}{\quad\forall}
\newcommand{\smallsum}{{\Sigma}}

\newcommand{\exclaim}{\char'041}

\newcommand{\globalf}{reduction}
\newcommand{\id}{$\langle${\sl id}$\rangle$ }
\newcommand{\expr}{$\langle${\sl expr}$\rangle$ }
\newcommand{\globalizd}{reducing}
\newcommand{\globalverb}{reduce}

\newcommand{\set}[2]{\left\lbrace #1 \; : \; #2 \right\rbrace}
\newcommand{\bigset}[2]{\big\lbrace #1 \; : \; #2 \big\rbrace}
\newcommand{\Bigset}[2]{\Big\lbrace #1 \; : \; #2 \Big\rbrace}
\newcommand{\Text}[1]{\;\hbox{#1}\;}
\newcommand{\qbox}[1]{\quad\hbox{#1}\quad}
\newcommand{\intbos}[1]{\oint_{\partial\Omega} #1 \, ds}
\newcommand{\bo}{{\partial\Omega}}
\newcommand{\intersect}{\cap}
\newcommand{\nullset}{\O}
\newcommand{\aRobin}{a_{{\rm Robin}}}
%\newcommand{\aRobin}{a_{\hbox{Robin}}}
\newcommand{\zbc}[1]{{\mathaccent"17  #1}}

\newcommand{\raqo}{{\cal R}}
\newcommand{\du}{{\cal D}(\uu)}
\newcommand{\duh}{{\cal D}(\uu_h)}
\newcommand{\dhu}{{\cal D}(\hat\uu)}
\newcommand{\dz}{{\cal D}(\zz)}
\newcommand{\dw}{{\cal D}(\ww)}
\newcommand{\dv}{{\cal D}(\vv)}
\newcommand{\dvz}{{\cal D}(\vv_0)}
\newcommand{\dvl}{{\cal D}(\vv_\lambda)}
\newcommand{\dchi}{{\cal D}(\bchi)}
\newcommand{\globalint}{{\cal I}_h}
\newcommand{\family}{{\cal T}_h}

\newcommand{\exporidsub}[1]{$<${\sl expr}$>_{#1}$ }
\newcommand{\synchronous}{{predictable}}
\newcommand{\asynchronous}{{chaotic}}
\newcommand{\commcomprat}{{work/memory ratio}}

\newfloat{code}{ht}{aux}[section]
\floatstyle{boxed}
\floatname{code}{Program}
\restylefloat{code}

\newcommand{\defdex}[1]{{\bf #1}\index{#1}} % use this for the word being defined 

\newcommand{\exursiz}[1]{Exercise~\ref{#1}}
\newcommand{\exursizstwo}[2]{Exercises~\ref{#1} and~\ref{#2}}
\newcommand{\pogram}[1]{Program~\ref{#1}}
\newcommand{\pogramstwo}[2]{Programs~\ref{#1} and~\ref{#2}}
\newcommand{\sexshun}[1]{Section~\ref{#1}}
\newcommand{\sexshunstwo}[2]{Sections~\ref{#1} and~\ref{#2}}
\newcommand{\sexshunsthree}[3]{Sections~\ref{#1},~\ref{#2} and~\ref{#3}}
\newcommand{\chaptur}[1]{Chapter~\ref{#1}}
\newcommand{\figgar}[1]{Figure~\ref{#1}}
\newcommand{\tabul}[1]{Table~\ref{#1}}
\newcommand{\Tabul}[1]{Table~\ref{#1}}
\newcommand{\defnn}[1]{Definition~\ref{#1}}
\def\emflab#1{{\em #1}\index{#1}}

\newcommand{\matlab}{{\tt octave}}
\newcommand{\albert}{albert}
\newcommand{\analysa}{{\tt Analysa}$_{{\rm \scriptscriptstyle TM}}$}
\newcommand{\postscript}{PostScript}

\newcommand{\intone}{\int_0^1}
\newcommand{\cpp}{C++}
\newcommand{\eqnn}[1]{(\ref{#1})}
%\newcommand{\eqnn}[1]{Equation~\ref{#1}}
\newcommand{\thmn}[1]{Theorem~\ref{#1}}
\newcommand{\lemn}[1]{Lemma~\ref{#1}}
\newcommand{\eqnntwo}[2]{Equations~\ref{#1} and \ref{#2}}
\newcommand{\eqnnthree}[3]{Equations~\ref{#1},~\ref{#2} and \ref{#3}}
\newcommand{\eqnnfour}[4]{Equations~\ref{#1},~\ref{#2},~\ref{#3} and \ref{#4}}
\newcommand{\dpd}[2]{{\partial{#1}\over\partial{#2}}}
\newcommand{\ddd}[2]{{d{#1}\over d{#2}}}
\newcommand{\pdo}[1]{{\partial\phantom{#1}\over\partial{#1}}}
\newcommand{\dpdm}[3]{{\partial^{#3}{#1}\over\partial{#2}^{#3}}}
\newcommand{\pdpnew}[2]{{\partial^{#2}{\phantom{1}}\over\partial #1^{#2}}}
\newcommand{\pdp}[2]{{\partial^{#2}{\phantom{#1}}\over\partial{#1}^{#2}}}
%\newcommand{\pdpf}[3]{{\partial^{#2}{#3}}\over\partial{#1}^{#2}}}

\newcommand{\Lones}{L^1(\Omega)}
\newcommand{\Ltos}{L^2(\Omega)}
\newcommand{\Ltbos}{L^2(\partial\Omega_h)}
\newcommand{\Lpos}{L^p(\Omega)}
\newcommand{\Lros}{L^r(\Omega)}
\newcommand{\Lqos}{L^q(\Omega)}
\newcommand{\Lios}{L^\infty(\Omega)}
\newcommand{\Hoos}{{H^1(\Omega)}}
\newcommand{\Hooz}{{H^1_0(\Omega)}}
\newcommand{\Hmoos}{{H^{-1}(\Omega)}}
\newcommand{\Htos}{{H^2(\Omega)}}
\newcommand{\Hmos}{{H^{m}(\Omega)}}
\newcommand{\Htoz}{\zbc{H}^2(\Omega)}
\newcommand{\Czio}{C_0^\infty(\Omega)}
\newcommand{\Woios}{W^1_\infty(\Omega)}
\newcommand{\Wopos}{W^1_p(\Omega)}
\newcommand{\norm}[1]{\Vert{#1}\Vert}
\newcommand{\dnorm}[1]{|{#1}|}
\newcommand{\seminorm}[1]{\vert{#1}\vert}
\newcommand{\Hoosn}[1]{\seminorm{#1}_{H^1(\Omega)}}
\newcommand{\tbnorm}[1]{\vert\kern-.1em\vert\kern-.1em\vert{\, #1 \,}\vert\kern-.1em\vert\kern-.1em\vert}
\newcommand{\Lto}[1]{\norm{#1}_{\Ltos}}
\newcommand{\Loneo}[1]{\norm{#1}_{\Lones}}
\newcommand{\Lpo}[1]{\norm{#1}_{\Lpos}}
\newcommand{\Lro}[1]{\norm{#1}_{\Lros}}
\newcommand{\Lqo}[1]{\norm{#1}_{\Lqos}}
\newcommand{\Lio}[1]{\norm{#1}_{\Lios}}
\newcommand{\Pinorm}[1]{\norm{#1}_{\Pi}}
\newcommand{\Hoo}[1]{\norm{#1}_{\Hoos}}
\newcommand{\Hmoo}[1]{\norm{#1}_{\Hmoos}}
\newcommand{\Hmo}[1]{\norm{#1}_{\Hmos}}
\newcommand{\Hmosn}[1]{\seminorm{#1}_{\Hmos}}
\newcommand{\Hmoosn}[1]{\seminorm{#1}_{\Hmoos}}
\newcommand{\Hto}[1]{\norm{#1}_{\Htos}}
\newcommand{\Htosn}[1]{\seminorm{#1}_{\Htos}}
%\newcommand{\Hdivs}{{H_{\rm div}(\Omega)}}
\newcommand{\Hdivs}{{H({\rm div};\Omega)}}
\newcommand{\Hdiv}[1]{\norm{#1}_{\Hdivs}}

\newcommand{\ut}[1]{{\bf #1}}
%\newcommand{\ut}[1]{\rlap{${}{\lower .2ex\hbox{$_{_\sim}$}}$}{#1}}
\newcommand{\utLt}{{L^2(\Omega)}}
%\newcommand{\utLt}{\rlap{${}{\lower .2ex\hbox{$_{_\sim}$}}$}{L^2}}
\newcommand{\dut}[1]{{\bf #1}}
%\newcommand{\dut}[1]{\rlap{${}{\lower .2ex\hbox{$_{_\sim}$}}$}{#1}}
%\newcommand{\dut}[1]{\rlap{${}{\lower .5ex\hbox{$_{_\approx}$}}$}{#1}}
%\newcommand{\Grad}{{\nabla \,}}
\newcommand{\oput}[1]{\rlap{${}{\lower 1.3ex\hbox{${\sim}$}}$}{#1}}
\newcommand{\Grad}{{\rm g\oput{\rm ra}d\,}}
\newcommand{\utVee}{{\bf V}}
%\newcommand{\utVee}{\rlap{${}{\lower .2ex\hbox{$_{_\sim}$}}$}{V}}
\newcommand{\dop}{{\mathcal D}}
\newcommand{\Div}{{\nabla\cdot \,}}
\newcommand{\grad}{{\nabla }}
\newcommand{\nosdiv}{{\nabla\cdot \,}}
\newcommand{\sdiv}{{{\nabla\cdot} \,}}
\newcommand{\curl}{{{\rm curl} \,}}
\newcommand{\bcurl}{{{\bf curl} \,}}
\newcommand{\diam}{\hbox{diam}}
%\newcommand{\sdiv}{{\oput{\nabla\cdot} \,}}
\newcommand{\proj}{{\cal P}}
\newcommand{\pieproj}{P_{\Pi}\,}
\newcommand{\pieprojh}{P_{\Pi_h}}
\newcommand{\R}{RR}
\newcommand{\teeh}{{\cal T}}
\newcommand{\goal}{{\cal M}}
%\newcommand{\th}{{\ca T}}
\newcommand{\polys}{{\cal P}}
\newcommand{\displfn}{{\cal P}}
\newcommand{\Pk}{{\polys_k}}
\newcommand{\Pkmo}{{\polys_{k-1}}}
%\def\interp{{\cal I}}
\newcommand{\interp}{{\cal I}}
\newcommand{\ext}{{\cal E}}
%%%%%%%%%%%%%%%%%%\newcommand{\bold}[1]{{\bf #1}}

\newcommand{\LI}{\lambda}
\newcommand{\MI}{\mu}
\newcommand{\RI}{\rho}
\newcommand{\LGI}{\iota}
\newcommand{\LGISET}{{\cal I}}
\newcommand{\Vspas}{{\cal V}}
\newcommand{\bldvr}[1]{{\bf #1}}
\newcommand{\dpdf}[2]{{\partial{#1}\over\partial{#2}}}

%\newenvironment{proof}{{\it Proof.}}{\hfill\qed\newline}

\newcommand{\ddt}{{\textstyle{d\phantom{t}\over dt}}}
\newcommand{\C}{{\mathbf C}}
\newcommand{\T}{{\mathbf T}}
\newcommand{\bfz}{{\mathbf 0}}
\newcommand{\rr}{{\mathbf r}}
\newcommand{\uu}{{\mathbf u}}
\newcommand{\bA}{{\mathbf A}}
\newcommand{\UU}{{\mathbf U}}
\newcommand{\VV}{{\mathbf V}}
\newcommand{\WW}{{\mathbf W}}
\newcommand{\XX}{{\mathbf X}}
\newcommand{\ZZ}{{\mathbf Z}}
\newcommand{\FF}{{\mathbf F}}
\newcommand{\vv}{{\mathbf v}}
\newcommand{\ww}{{\mathbf w}}
\newcommand{\zz}{{\mathbf z}}
\newcommand{\gbc}{{\mathbf g}}
\newcommand{\ba}{{\mathbf a}}
\newcommand{\bt}{{\mathbf t}}
\newcommand{\nn}{{\mathbf n}}
\newcommand{\ff}{{\mathbf f}}
\newcommand{\xx}{{\mathbf x}}
\newcommand{\ee}{{\mathbf e}}
\newcommand{\yy}{{\mathbf y}}
\newcommand{\intox}[1]{\int_{\Omega} #1 \, d\xx}
\newcommand{\inty}[1]{\int_0^\infty #1 \, dy}
\newcommand{\intoxl}[1]{\int_{\Omega_L} #1 \, dx\, dy\, dz}
\newcommand{\intoxz}[1]{\int_{\Omega_0} #1 \, dx\, dy\, dz}
\newcommand{\intoxt}[1]{\int_{\Omega} #1 \, dx\, dy}
\newcommand{\tant}{{\mathbf t}}

\newcommand{\dpdtu}[1]{\frac{d^2{\phantom{#1}}}{d{#1}^2}}
\newcommand{\dpdo}[1]{\frac{\partial{\phantom{#1}}}{\partial{#1}}}
\newcommand{\tps}{{t}}
\newcommand{\bepsilon}{{\boldsymbol \epsilon}}
\newcommand{\eps}{{\epsilon}}
\newcommand{\beps}{{\boldsymbol \eps}}
\newcommand{\bphi}{{\boldsymbol \phi}}
\newcommand{\bxi}{{\boldsymbol \xi}}
\newcommand{\bpsi}{{\boldsymbol \psi}}
\newcommand{\bchi}{{\boldsymbol \chi}}
\newcommand{\bbeta}{{\boldsymbol \beta}}
\newcommand{\balpha}{{\boldsymbol \alpha}}
\newcommand{\bgamma}{{\boldsymbol \gamma}}
\newcommand{\bzeta}{{\boldsymbol \zeta}}
\newcommand{\bomega}{{\boldsymbol \omega}}

\newcommand{\deltat}{\Delta t}
\newcommand{\datekern}{{\relax\kern+.1em}--{\relax\kern-.01em}}

\newcommand{\centr}[1]{\begin{center} {#1} \end{center}}
\newcommand\bigforall{\mbox{\Large $\mathsurround0pt\forall$}}
\newcommand{\antiparallel}{\not\kern-0.35em\Vert}

\newcommand{\derdir}[2]{{\frac{\partial{#1}}{\partial #2}}}
\newcommand{\bdtuh}{u^*_h}
\newcommand{\ruh}{\hat u_h}
\newcommand{\dceps}{{\small\mathcal E}}
%\newcommand{\dceps}{\varepsilon}
\newcommand{\order}[1]{{\cal O}\left(#1\right)}

\newcommand{\Reno}{{\hbox{\tiny\rm Re}}}
\newcommand{\argmin}{\hbox{\rm argmin}}
\newcommand{\mybox}[1]{{\fbox{$\displaystyle #1$}}}
\newcommand{\solushun}[1]{\section{\, Solution of Exercise \ref{#1}}\par\smallskip}
%\newcommand{\solushun}[1]{\section{\;\rm Solution of Exercise \ref{#1}}\par\smallskip}
%\newcommand{\solushun}[1]{\section{\;\bf Solution of Exercise \ref{#1}}\par\smallskip}
%\newcommand{\solushun}[1]{{\bf Solution of Exercise \ref{#1}}\par\smallskip}
\newcommand{\fural}{{\quad\hbox{for all}\;}}
\newcommand{\sech}{{\hbox{sech}}}

